Soft interaction model and the LHC data

Most models for soft interactions which were proposed prior to the measurements at the LHC, are only marginally compatible with LHC data, our GLM model has the same deficiency. In this paper we investigate possible causes of the problem, by considering separate fits to the high energy ($W > 500\, GeV$), and low energy ($W < 500\, GeV$) data. Our new results are moderately higher than our previous predictions. Our results for total and elastic cross sections are systematically lower that the recent Totem and Alice published values, while our results for the inelastic and forward slope agree with the data. If with additional experimental data, the errors are reduced, while the central cross section values remain unchanged, we will need to reconsider the physics on which our model is built.

==> nflhc-ref.tex <==
\begin{thebibliography}{99}
\bibitem{ALICE}
M.~G.~Poghosyan,
  %``Diffraction dissociation in proton-proton collisions at $\sqrt{s}$ = 0.9 TeV, 2.76 TeV and 7 TeV with ALICE at the LHC,''
  J.\ Phys.\ G G {\bf 38}, 124044 (2011)
  [arXiv:1109.4510 [hep-ex]].
 ALICE ~Collaboration,
  {\it ``First proton--proton collisions at the LHC as observed with the ALICE
  detector: measurement of the charged particle pseudorapidity density at
  $\sqrt{s}$ = 900 GeV,''}
  arXiv:0911.5430 [hep-ex].
  %%CITATION = ARXIV:0911.5430;%%
  %%CITATION = ARXIV:1109.4510;%%
\bibitem{ATLAS}
G.~Aad {\it et al.}  [ATLAS Collaboration],
  %``Measurement of the Inelastic Proton-Proton Cross-Section at $\sqrt{s}=7$ TeV with the ATLAS Detector,''
  Nature Commun.\  {\bf 2} (2011) 463
  [arXiv:1104.0326 [hep-ex]].
  %%CITATION = ARXIV:1104.0326;%%
\bibitem{CMS}
CMS Physics Analysis Summary:
Measurement of the inelastic pp cross section at √s = 7 TeV with the CMS detector", 2011/08/27./


\bibitem{TOTEM}
 F.~Ferro [TOTEM Collaboration],
  %``First data from TOTEM experiment at LHC,''
  AIP Conf.\ Proc.\  {\bf 1350} (2011) 172;\,\,\,G.~Antchev {\it et al.}  [TOTEM Collaboration],
  %``First measurements of the total proton-proton cross section at the LHC energy of \sqrt s =7TeV,''
  Europhys.\ Lett.\  {\bf 96} (2011) 21002,
  %``Proton-proton elastic scattering at the LHC energy of s** (1/2) = 7-TeV,''
  {\bf 95} (2011) 41001
  [arXiv:1110.1385 [hep-ex]].
  %%CITATION = ARXIV:1110.1385;%%
  %%CITATION = APCPC,1350,172;%%


  %%CITATION = EPHJA,C57,689;%%
\bibitem{GLM}
 E.~Gotsman, E.~Levin and U.~Maor,
  %``N=4 SYM and QCD motivated approach to soft interactions at high energies,''
  Eur.\ Phys.\ J.\  C {\bf 71} (2011) 1553
  [arXiv:1010.5323 [hep-ph]];
  \,\,\,  E.~Gotsman, E.~Levin, U.~Maor and J.~S.~Miller,
  %``A QCD motivated model for soft interactions at high energies,''
  Eur.\ Phys.\ J.\  C {\bf 57} (2008) 689
  [arXiv:0805.2799 [hep-ph]].
  %%CITATION = EPHJA,C71,1553;%%
\bibitem{KAP}
 A.~B.~Kaidalov and M.~G.~Poghosyan,
  %``Description of soft diffraction in the framework of reggeon calculus.
  %Predictions for LHC,''
  arXiv:0909.5156 [hep-ph].
  %%CITATION = ARXIV:0909.5156;%%

\bibitem{KMR}
 A.~D.~Martin, M.~G.~Ryskin and V.~A.~Khoze,
  %``From hard to soft high-energy pp interactions,''
  arXiv:1110.1973 [hep-ph].
  %%CITATION = ARXIV:1110.1973;%%
\bibitem{OST}
S.~Ostapchenko,
  %``Monte Carlo treatment of hadronic interactions in enhanced Pomeron scheme:
  %I. QGSJET-II model,''
  Phys.\ Rev.\  D {\bf 83} (2011) 014018
  [arXiv:1010.1869 [hep-ph]].
  %%CITATION = PHRVA,D83,014018;%%

.
\bibitem{BST}
 R.~C.~Brower, J.~Polchinski, M.~J.~Strassler and C.~I.~Tan,
  %``The Pomeron and Gauge/String Duality,''
  JHEP {\bf 0712} (2007) 005
  [arXiv:hep-th/0603115];\,\,
  %%CITATION = JHEPA,0712,005;%%
R. C. Brower, M. J. Strassler and C. I. Tan,
{\it "On The Pomeron at Large 't Hooft Coupling"}, arXiv:0710.4378 [hep-th].
 \bibitem{HIM}
Y.~Hatta, E.~Iancu and A.~H.~Mueller,
  %``Deep inelastic scattering at strong coupling from gauge/string duality :
  %the saturation line,''
  JHEP {\bf 0801} (2008) 026
  [arXiv:0710.2148 [hep-th]].
  %%CITATION = JHEPA,0801,026




 \bibitem{COCO}
 L.~Cornalba and M.~S.~Costa,
  %``Saturation in Deep Inelastic Scattering from AdS/CFT,''
 Phys. Rev. {\bf D 78}, (2008) 09010,
  arXiv:0804.1562 [hep-ph];\,\,\,
  L.~Cornalba, M.~S.~Costa and J.~Penedones,
  %``Eikonal Methods in AdS/CFT: BFKL Pomeron at Weak Coupling,''
  JHEP {\bf 0806} (2008) 048
  [arXiv:0801.3002 [hep-th]];\,\,
  %``Eikonal Approximation in AdS/CFT: Resumming the Gravitational Loop
  %Expansion,''
  JHEP {\bf 0709} (2007) 037
  [arXiv:0707.0120 [hep-th]].
  %%CITATION = JHEPA,0709,037;%%
  %%CITATION = JHEPA,0806,048;%%
    %%CITATION = ARXIV:0804.1562;%%

\bibitem{BEPI}
B.~Pire, C.~Roiesnel, L.~Szymanowski and S.~Wallon,
  %``On AdS/QCD correspondence and the partonic picture of deep inelastic
  %scattering,''
  Phys.\ Lett.\  B {\bf 670}, 84 (2008)
  [arXiv:0805.4346 [hep-ph]].
  %%CITATION = PHLTA,B670,84;%%
\bibitem{LMKS}
E.~Levin, J.~Miller, B.~Z.~Kopeliovich and I.~Schmidt,
 % {\it ``Glauber - Gribov approach for DIS on nuclei in N=4 SYM,''}
JHEP {\bf 0902} (2009) 048;\,\,
  arXiv:0811.3586 [hep-ph].
  %%CITATION = ARXIV:0811.3586;


  \bibitem{LEPO}
  R.~C.~Brower, M.~Djuric, I.~Sarcevic, C.~-ITan,
  %``String-Gauge Dual Description of Deep Inelastic Scattering at Small-$x$,''
  JHEP {\bf 1011 } (2010)  051.
  [arXiv:1007.2259 [hep-ph]];\,\,\,
 E.~Levin, I.~Potashnikova,
  %``Inelastic processes in DIS and N=4 SYM,''
  JHEP {\bf 1008 } (2010)  112.
  [arXiv:1007.0306 [hep-ph]]

\bibitem{GW}
M. L. Good and W. D. Walker,
Phys. Rev. {\bf 120} (1960) 1857.
\bibitem{MPSI}
A. H. Mueller and B. Patel,
Nucl. Phys. {\bf B425} (1994) 471. 
A. H. Mueller and G. P. Salam,
Nucl. Phys. {\bf B475}, (1996) 293. [arXiv:hep-ph/9605302]. 
G. P. Salam,
Nucl. Phys. {\bf B461} (1996) 512; 
E. Iancu and A. H. Mueller,
Nucl. Phys. {\bf A730} (2004) 460 [arXiv:hep-ph/0308315];            
494 [arXiv:hep-ph/0309276].
\bibitem{RY}
I. Gradstein and I. Ryzhik, 
{\it "Tables of Series, Products, and Integrals"}, Verlag MIR, Moskau,1981.
\bibitem{AGK}
 ~V.~A. Abramovsky, V.~N.~ Gribov,V.~N.~ and  O.~V.~ Kancheli,
 % Character of inclusive spectra and fluctuations produced in inelastic procesesses by multi-Pomeron exchange,
 Sov.\ J.\ Nucl.\ Phys.\,{\bf 18} (1973) 308,
[Yad.\ Fiz.\,{\bf 18} (1973) 595].


\bibitem{PDG}
C. Amsler et al. (Particle Data Group), Physics Letters, {\bf  B667}  (2008) 1. 

\bibitem{KMW}
 H. Kowalski, L. Motyka and G. Watt, Phys. Rev.{\bf  D 74}  (2006) 074016. [arXiv:hep-ph/0606272].
\bibitem{H1ZEUSlam}
%\cite{Adloff:2000qk}
%\bibitem{Adloff:2000qk}
  C.~Adloff {\it et al.}  [H1 Collaboration],
  %``Deep-inelastic inclusive e p scattering at low x and a determination of
  %alpha(s),''
  Eur.\ Phys.\ J.\  C {\bf 21} (2001) 33;
  [arXiv:hep-ex/0012053].
  %%CITATION = EPHJA,C21,33;%%

%\cite{Chekanov:2001qu}
%\bibitem{Chekanov:2001qu}
  S.~Chekanov {\it et al.}  [ZEUS Collaboration],
  %``Measurement of the neutral current cross section and F2 structure  function
  %for deep inelastic e+ p scattering at HERA,''
  Eur.\ Phys.\ J.\  C {\bf 21} (2001) 443.
  [arXiv:hep-ex/0105090].
  %%CITATION = EPHJA,C21,443;%%
\bibitem{HERAFIT}
$https://www.desy.de/h1zeus/combined_results/herapdftable.html;
http://hepdata.cedar.ac.uk/pdf/pdf3.html;$

\bibitem{CUD}
 Cudell J. et al., Phys. Rev. Lett., 89 (2002) 201801.
\bibitem{BLHA}
M.~Block and F.~Halzen.
Phys. Rev. Lett. {\bf 107} 212002 (2011).
\bibitem{ATLASSD}
 A.~Collaboration,
  %``Rapidity gap cross sections measured with the ATLAS detector in pp collisions at sqrt(s) = 7 TeV,''
  arXiv:1201.2808 [hep-ex].
  %%CITATION = ARXIV:1201.2808;%%
\bibitem{GLMSP}
  E.~Gotsman, E.~Levin and U.~Maor,
  %``Survival probability of large rapidity gaps in QCD and N=4 SYM motivated model,''
  Eur.\ Phys.\ J.\ C {\bf 71} (2011) 1685
  [arXiv:1101.5816 [hep-ph]].
  %%CITATION = ARXIV:1101.5816;%%
  \bibitem{E710}
E710 Collaboration, Phys. Lett. B247 (1990) 127;\\
 CDF Collaboration, Phys. Rev. D50 (1994) 5518.
 
 \bibitem{RISTO}
R. Orava, Talk at Workshop:{\it `` Exclusive and diffractive processes in high energy proton-proton and nucleus-nucleus collisions"}, February 27 - March 2 , 2012, Trento, Italy;
http://diff2012-lhc.physi.uni-heidelberg.de/Talks/orava.pdf


\end{thebibliography}


